SafeEar: Content Privacy-Preserving Audio Deepfake Detection

Text-to-Speech (TTS) and Voice Conversion (VC) models have exhibited remarkable performance in generating realistic and natural audio. However, their dark side, audio deepfake poses a significant threat to both society and individuals. Existing countermeasures largely focus on determining the genuineness of speech based on complete original audio recordings, which however often contain private content. This oversight may refrain deepfake detection from many applications, particularly in scenarios involving sensitive information like business secrets. In this paper, we propose SafeEar, a novel framework that aims to detect deepfake audios without relying on accessing the speech content within. Our key idea is to devise a neural audio codec into a novel decoupling model that well separates the semantic and acoustic information from audio samples, and only use the acoustic information (e.g., prosody and timbre) for deepfake detection. In this way, no semantic content will be exposed to the detector. To overcome the challenge of identifying diverse deepfake audio without semantic clues, we enhance our deepfake detector with real-world codec augmentation. Extensive experiments conducted on four benchmark datasets demonstrate SafeEar's effectiveness in detecting various deepfake techniques with an equal error rate (EER) down to 2.02%. Simultaneously, it shields five-language speech content from being deciphered by both machine and human auditory analysis, demonstrated by word error rates (WERs) all above 93.93% and our user study. Furthermore, our benchmark constructed for anti-deepfake and anti-content recovery evaluation helps provide a basis for future research in the realms of audio privacy preservation and deepfake detection.

==> sections/design.tex <==
% !TEX ROOT =../main.tex
\section{Design Details}\label{sec:design}
% 1. why we can preserve the privacy? an intuitive case
% 2. why the lack of content features should not significantly affect the spoofing detection performance?
% 3. We can conduct preliminary experiments as ``Silence is Gold'', which validates the 
% 4. Display three spectrums in the forms of ``original speech'', ``semantic-only speech'', and ``acoustic-only speech''  %比如能够证明mfcc等特征存在很容易被复原的信息。
\subsection{Overview of \sys}\label{ssec:design_overview}
% \subsection{\sys's Idea and Intuition}\label{ssec:design_overview}
\hspace{0.4cm}\textbf{Key Idea.} We aim to propose a framework that achieves two seemingly contradictory objectives: effective deepfake detection and prevention of any attempts at content recovery. Our key idea is to design a novel frontend feature extractor that can decompose speech information into mutually independent discrete representations, \textit{i.e.}, semantic and acoustic tokens, where only the latter being analyzed by subsequent deepfake detectors. Such acoustic tokens can enable effective deepfake detection, but nullify recovery attempts by both machine and human auditory analysis.

\textbf{Intuition Behind \sys.}
The idea of \sys is rooted in a critical insight: audio deepfake technology primarily concentrates on capturing the unique vocal attributes of a target speaker, such as timbre, loudness, rhythm, and pitch, which constitute acoustic information~\cite{liu2023unifyspeech}. However, this technology typically overlooks the actual speech content. %Therefore, deepfake detection shall pivot towards acoustic information. 
In fact, several studies have already confirmed the significance of acoustic features in detecting deepfake audios, \textit{e.g.}, timbre~\cite{chaiwongyen2022contribution}, pitch and loudness~\cite{li2022comparative}. In contrast, the core of speech comprehension, both in humans and as modeled in ASR systems, lies in accurately transcribing the semantic content, irrespective of variations in the speaker's acoustic patterns~\cite{yasmin2023effects}. 
% This perspective is further supported by a recent research, which found that acoustic and semantic information are highly independent. 
The above understanding leads us to believe that developing a deepfake audio detector merely based on acoustic information is feasible. Acoustic information's devoid of semantic content exploitable by adversaries, inherently preserves content privacy.


\textbf{Challenges}. To realize \sys, we faces two challenges. \textit{Challenge 1}: How to design a novel decoupling module that well extracts and secures acoustic tokens, protecting speech content from recovery by machine and human auditory analysis? \textit{Challenge 2}: How to ensure reliable detection against various real-world deepfake audio, despite relying solely on acoustic tokens?
% Finally, Challenge 4 (C4) focuses on validating the system through a comprehensive benchmark that includes both standard datasets and our own larger dataset to test the detection and protection capabilities of the system.


\textbf{Methodology Outline}. 
As shown in Figure~\ref{fig:fig3}, to address \textit{Challenge 1}, we carefully devise a neural codec architecture (\S\ref{sec:CDM}, \ding{172} in Figure~\ref{fig:fig3}) to flexibly decompose the audio signal $\mathbf{X}\in \mathbb{R}^{1\times T}$ into semantic tokens $\mathbf{S}\in \mathbb{R}^{C\times T_n}$ and acoustic tokens $\mathbf{A}\in \mathbb{R} ^{7C\times T_n}$, where $C$ denotes the token dimension, and $T$ and $T_n$ represent the length of the audio and token, respectively. We combine a bottleneck and shuffle layer (\S\ref{sec:shuffle}, \ding{173} in Figure~\ref{fig:fig3}) to secure the tokens as $\mathbf{\overline{A}}\in \mathbb{R}^{C\times T_n}$, thereby the original content cannot be reconstructed. For \textit{Challenge 2}, we finely tune our backend detector (\S\ref{ssec:design_detection}, \ding{174} in Figure~\ref{fig:fig3}) with optimal number of self-attention heads, as well as mimicking real-world codec transformation from $\mathbf{X}$ to $\mathbf{X^*}$ for the detector training (\S\ref{ssec:codec_augment}, \ding{175} in Figure~\ref{fig:fig3}).
% For C4, we introduce a wide range of benchmarks (\S\ref{sec:Benchmark}), including standard datasets from challenges such as ASVspoof 2019~\cite{ASVspoof2019_dataset} and ASVspoof 2021~\cite{ASVspoof2021_dataset}, as well as a large dataset we have developed ourselves to provide a strong validation of \sys' capabilities.

% The architecture of \sys is demonstrated in Figure~\ref{fig:fig3}. The core of this architecture employs a decoupling approach based on neural codecs to flexibly decompose the audio signal for semantic anonymization, which facilitates the detection of deepfake audio. At the first stage, the neural codec decomposes the input speech signal $\mathbf{X}\in \mathbb{R}^{1\times T}$ into semantic tokens $\mathbf{S}\in \mathbb{R}^{C\times T_n}$ and acoustic tokens $\mathbf{A}\in \mathbb{R} ^{7C\times T_n}$, where $C$ denotes the token dimension, and $T$ and $T_n$ represent the length of the audio and token, respectively. Next, the acoustic features are tuned in the bottleneck and shuffle layers to prevent the attacker from reconstructing the original content. Eventually, these enhanced features $\mathbf{\overline{A}}\in \mathbb{R}^{C\times T_n}$ are fed into the backend detector (i.e., the classification network) for distinguishing between bonafide and deepfake audio.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/design_overview2.pdf}
    \caption{Overview of the \sys framework. In the inference phase, we just need to remove \ding{175}.}
    \label{fig:fig3}
\end{figure}

\subsection{Codec-based Decoupling Model (CDM)}\label{sec:CDM}
% 这里需要体现为什么我们选择codec-based，而不是其他？(因为codec本身就在各种实时通信平台上使用)
% As depicted in Figure~\ref{fig:CDM}, the Codec-based Decoupled Model (CDM) consists of three main modules: encoder, residual vector quantizer (RVQ), and decoder. 
% \hspace{0.4cm}\textbf{Motivation of Neural Codec-based Decoupling.} 

% 2024.1.24 还得点出来我们用discriminator的好处是能够保证语音质量，因为codec本身就在virtual通信中使用；另外不要太强调encodec，这样就会被迫跟它的语音质量进行对比？
% 下文更多是体现一个如何做到声学和语义的解缠
% As neural codecs' inherent usage for virtual communications, prior works~\cite{Encodec,Soundstream} largely focus using decoder to reconstruct RVQs Different from prior works that focus on , we aim to 
Inspired by the recent paradigm in neural audio codecs like Encodec~\cite{Encodec} and Soundstream~\cite{wang2023neural}, which leverage the multi-layer residual vector quantizers (RVQs)~\cite{van2017neural} to accurately represent speech with discrete speech tokens for high-quality and efficient audio transmission in a sound type- and language-agnostic manner\footnote{More description of audio codecs are provided in Appendix~\ref{ssec:audio_codec}.}.
% Given that the inherent use of neural codec in virtual calls, where audio deepfake can also happen. 
We aim to develop the neural codec architecture into an effective decoupling model that separates mixed speech tokens into standalone semantic and acoustic tokens.
As illustrated in Figure~\ref{fig:CDM}, our proposed decoupling model based on the codec architecture (CDM) comprises three core components: an encoder, a HuBERT-equipped RVQs module, and a discriminator-enhanced decoder. The encoder is responsible for extracting key features from speech signals, the HuBERT-equipped RVQs further decouple these features and hierarchically quantize them into discrete semantic and acoustic tokens, and the discriminator-enhanced decoder reconstructs original signals from these discrete tokens. Through this structure, we can achieve effective decoupling of speech signals. The decoupled semantic and acoustic audio samples can be found in our demo page~\cite{safeear_demo}.  % data without compromising speech quality.

% \textbf{Encoder}. To decompose the speech signal $\mathbf{X}$, the CDM first passes through a series of consecutive convolutional layers to obtain the embedding feature $\mathbf{E}\in \mathbb{R}^{C\times T_n}$. In the encoder, we employ $D$ downsampling modules, each consisting of a one-dimensional convolutional layer with $C$ channels and a kernel size 7, immediately followed by $M$ residual convolutional modules. Each residual convolution module consists of two convolutional layers with kernel sizes of 3 and 1, respectively. In addition, a one-dimensional convolutional layer with kernel size $K$ and step size $K/2$ is used for the downsampling layer. During each downsampling process, the number of channels is doubled, and each convolutional layer is followed by an exponential linear unit (ELU) and layer normalization. Finally, the semantic modeling capability of the encoder is enhanced by BiLSTM to obtain the embedded feature $\mathbf{E}$.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/design_frontend.pdf}
    \caption{Frontend codec-based decoupling model (\ding{172}) of \sys.}
    \label{fig:CDM}
    \vspace{-10pt}
\end{figure}

\textbf{Encoder}. To efficiently extract information-rich features $\mathbf{E}\in \mathbb{R}^{C\times T_n}$ from the raw audio $\mathbf{X}$, we employ $D$ downsampling modules in the encoder architecture. Each downsampling module contains a one-dimensional convolutional layer of $C$ channels and a 7-sized kernel, followed by $M$ residual convolutional modules for detailed speech signal capture. During downsampling, the number of channels is progressively doubled, and we use the exponential linear unit (ELU) with layer normalization in each convolutional layer to enhance the nonlinear representation and stability of the model. Finally, to enhance the capability of semantic modelling, we integrate a bidirectional long and short-term memory network (Bi-LSTM) to more accurately capture the semantic and acoustic information in the audio feature space. This design helps to improve the performance of RVQs feature decoupling.

\textbf{HuBERT-equipped RVQs for Decoupling.}
% \red{Necessary to convey a detail of our design that facilitates the cross-language decoupling, \textit{i.e.}, the RVQ-1 inherently takes the main information, so that despite our supervising signal does not take the non-English corpus into account. SafeEar can also retains primary information in the RVQ-1 and the RVQ2:8 mainly describes speech details}
% For the output of the encoder, we employ a Residual Vector Quantizer (RVQ) for quantization processing. Specifically, the input vector is projected onto a predefined-sized codebook, and the nearest code is selected as the quantized representation. The RVQ includes $Q$ layers of cascaded Vector Quantization (VQ), aimed at mitigating the trade-off between the size of the codebook and quantization performance. Initially, the unquantized input vector passes through the first quantizer, generating a quantized residual $\mathbf{z_i}\in \mathbb{R}^{C\times T_n}$. Subsequently, these residuals are iteratively quantized through the remaining $Q-1$ quantizers. For each residual step $\{i \in {1,\dots, N_q}\}$, $\mathbf{z_i}$ represents the vector before quantization, and $q(\mathbf{z_i})$ represents the vector after quantization. To decouple the features of the encoder's output in RVQ, we divide RVQ into semantic and acoustic tokens. In the semantic token part, the first quantizer is used for semantic guidance to capture content information. Specifically, the tokens outputted by the first quantizer are decoupled from the audio content information through knowledge distillation with the average features $\mathbf{H}\in \mathbb{R}^{C\times T_n}$ of all HuBERT layers \cite{hsu2021hubert}. In the acoustic token part, the semantic token is subtracted from the output features of the encoder to obtain acoustic features devoid of content information, which are further extracted through seven quantizers. Finally, the output of all quantizers is accumulated to form the input for the decoder, which is used to reconstruct the original audio.
In CDM, we utilize Residual Vector Quantizers (RVQs) to effectively decouple semantic and acoustic tokens from the output of the encoder $\mathbf{E}$. The RVQs employ cascaded vector quantization (VQ) layers, which project the input vector onto a predefined codebook to obtain a quantized representation. 
% This approach is designed to balance the codebook size and the quantization performance. 
% To decouple the features of the encoder's output in RVQ, we divide RVQ into semantic and acoustic tokens. 
% To explicitly enhance the decoupling, we divide the RVQs into two parts: the semantic token part (VQ1) and the acoustic token part (VQ2:8).
% In the semantic token part, the first quantizer is used for semantic guidance to capture content information. Specifically, the tokens output by the first quantizer is decoupled from the speech content information through knowledge distillation with the average features $\mathbf{H}\in \mathbb{R}^{C\times T_n}$ of all HuBERT layers~\cite{hsu2021hubert}. In the acoustic token part, the semantic token is subtracted from the output features of the encoder to obtain acoustic features devoid of content information, which are further extracted through seven quantizers. Finally, the output of all quantizers is accumulated to form the input for the decoder, which is used to reconstruct the original audio.
To effectively achieve decoupling, we have specifically designed and adjusted the RVQs, dividing it into two main parts: the semantic token part (VQ1) and the acoustic token part (VQ2$\sim$VQ8). 

In the semantic token part, we aim to modify the first quantizer (VQ1) to capture the semantic information from speech, serving a content-centric role. Specifically, we introduce a knowledge distillation approach, \textit{i.e.}, employing the well-established HuBERT~\cite{hsu2021hubert} as our semantic teacher of VQ1. Since HuBERT can well represent given speech as semantic-only features~\cite{mohamed2022self}, we employ the average representation across all HuBERT layers as the semantic supervision signal that encourages the semantic student VQ1 to learn a very close content representation via:
\begin{equation}\label{eq:distilliation}
    \mathcal{L}_{distll}=\frac{1}{T_n}\sum_{t=1}^{T_n}\log\sigma(\cos{(\mathbf{W}\cdot\mathbf{S}_t,\mathbf{H}_t)})
\end{equation}
% \begin{equation}\label{eq:distilliation}
%     \mathcal{L}_{\text{distll}}=\log \sigma\left(\cos \left(\mathbf{W} \cdot q(\mathbf{z_1} ), \mathbf{H} \right)\right),
% \end{equation}
% where $q(\mathbf{z}_1)$ represents the output of the first VQ layer, $\mathbf{H}\in \mathbb{R}^{C\times T_n}$ denotes the mean of the output features of all HuBERT layers, $\cos(\cdot)$ signifies the cosine similarity between two variables, and $\mathbf{W}$ is the projection matrix.
where $\mathbf{S}_t$ and $\mathbf{H}_t$ respectively denote the $t^{th}$ quantized output, \textit{i.e.},  $t^{th}$ token frame of the VQ1 and the HuBERT. $\cos(\cdot)$ is cosine similarity. $\sigma(\cdot)$ denotes sigmoid activation. $\mathbf{W}$ is the projection matrix.


Subsequently, in the acoustic token part, VQ1's semantic tokens $\mathbf{S}$ will be stripped away from the full-information encoder's output $E$, resulting in purified acoustic information devoid of semantic information. These features are then passed to the subsequent seven quantizers (VQ2$\sim$VQ8), each further refining the acoustic information to enhance the feature representation of the sound. Through this layered and progressively refined processing, RVQs can handle complex sound data more efficiently. Ultimately, the outputs of all quantizers (VQ1$\sim$VQ8) are accumulated to form the input for the decoder. This accumulation process effectively recombines the semantic and acoustic information, enabling the decoder to reconstruct the original audio accurately. This design allows RVQs to effectively decouple audio content's semantic and acoustic properties while maintaining efficient encoding.
Please note that our design facilitates the cross-language decoupling, \textit{i.e.}, the VQ1 inherently takes the main information, so that despite our ``semantic teacher'' signal does not take the non-English corpus into account. \sys can also retain primary information in the VQ1 and the VQ2$\sim$VQ8 mainly describe speech details.

\textbf{Discriminator-enhanced Decoder.}
We utilize the decoder in our model because it is essential for reconstructing the decoupled semantic and acoustic tokens into the original audio. This part is key to produce an output that closely resembles the original audio signal, thereby maintaining the integrity and accuracy of the speech representation. Without the decoder, the acoustic tokens from the RVQs may not be able to achieve an accurate representation of the corresponding original audio. This is due to the potential inaccuracies in training an Encoder-Decoder pair. In our design, the decoder mirrors the structure of the encoder, but in reverse. 
% Consequently, it can precisely reconstruct any given tokens into audio waveforms. 
To enhance the audio quality reconstructed by our decoder, we have integrated three discriminators: the multiscale short-time Fourier transform (MS-STFT)~\cite{kumar2019melgan}, the multiperiodic (MPD), and the multiscale (MSD)~\cite{defossez2022high} discriminators. The MS-STFT discriminator analyzes complex-valued multiscale STFTs to capture detailed audio signal features. In contrast, the MPD and MSD focus on the periodic elements and long-term patterns in the audio. These discriminators employ various sub-discriminators to analyze audio samples of different sizes and segments, ensuring the accuracy and integrity of the reconstructed audio.


% To enhance the audio reconstructed by the decoder, we integrate three discriminators: the multiscale short-time Fourier transform (MS-STFT)~\cite{kumar2019melgan}, the multiperiodic (MPD) and the multiscale (MSD)~\cite{defossez2022high} discriminators. The MS-STFT analyses the complex-valued multiscale STFTs using multiple networks to capture the audio signal features. The MPD and the MSD are borrowed from HiFiGAN \cite{defossez2022high}, focusing on periodic elements and long-term patterns in audio. The MPD uses sub-discriminators for different audio sample segments, while the MSD uses three sub-discriminators to evaluate different sizes of audio input. MPD uses sub-discriminators for different audio sample segments, while MSD uses three sub-discriminators to evaluate audio inputs of different sizes.


% \textbf{Discriminator}. To enhance the quality of the generated samples, we adopt an integrated discriminator strategy that combines the multiscale short-time Fourier transform discriminator (MS-STFT), the multiperiodic discriminator (MPD), and the multiscale discriminator (MSD) for a more detailed loss computation. The MS-STFT discriminator \cite{kumar2019melgan} uses multiple structurally identical sub-networks that operate on the complex-valued multiscale STFT that connect the real and imaginary parts to capture different structural features in the audio signal. Each sub-network consists of a 2D convolutional layer followed by an incremental dilation rate 2D convolution in the time dimension. The final 2D convolutional layer with a kernel size of $3\times 3$ and a step size of $1\times 1$ is used to output the final prediction. MPD and MSD, on the other hand, use similar configurations to HiFiGAN \cite{defossez2022high}, dealing with periodic components of the input audio and capturing continuous patterns and long-term dependencies, respectively. MPD consists of multiple sub-discriminators, each dealing with equally spaced samples of the input audio, whereas MSD evaluates the continuity of the audio sequences. MSD consists of three sub-discriminators operating on inputs of different sizes: original audio, $\times 2$ and $\times 4$ average pooled audio. Each sub-discriminator of the MSD consists of a stack of hierarchical and grouped convolutional layers using a LeakyReLU activation function, which scales the discriminator by decreasing the span and increasing the number of layers.

\subsection{Bottleneck \& Shuffle Layer}\label{sec:shuffle}
As shown in Figure~\ref{fig:shuffle}, the frontend CDM of \sys initially encodes waveform inputs into discrete acoustic tokens, $\mathbf{A}$, with each frame denoted as $\mathbf{A}_i$. The bottleneck layer aims to reduce the dimensions of acoustic tokens $\mathbf{A}$ from $\mathbb{R}^{7C\times T_n}$ to a more compact space $\mathbf{A}^{b} \in \mathbb{R}^{C\times T_n}$ by using 1D convolution and batch normalization. This layer serves a dual purpose: first, it enhances computational efficiency and reduces trainable parameters, faciliating subsequent layers to operate on a compact representation; second, it acts as a regularizer, avoiding over-fitting by limiting the amount of acoustic tokens and stabilizing it via batch normalization, before analyzed by the deepfake detector.

In addition to decoupling speech information, the shuffle layer serves to augment content protection by further scrambling the condensed acoustic tokens $\mathbf{A}^{b}$. As shown in Figure~\ref{fig:shuffle}, By randomly rearranging the elements across the temporal dimension $T_n$, this layer nullifies speech comprehension that is highly dependent on the temporal order of phonemes and words~\cite{Nature_contextual}. We empirically set a shuffling window of 1 second, corresponding to 50 frames, to obscure word-level intelligibility (as each token representation is extracted from a 20ms waveform). \blue{Thereby, the likelihood of attackers deciphering and correcting these sequences is extremely low, given the sheer number of possible permutations for a 4-second audio ($50!^4$, approximately $8.56 \times 10^{257}$, details are discussed in \S\ref{sec:disucssion})}. Our experiments also confirm the dual content protection by decoupling and shuffling, thwarting the advanced ASR techniques and human auditory analysis.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/design_shuffle2.pdf}
    \caption{Bottlneck \& Shuffle layers (\ding{173}) of \sys.}
    \label{fig:shuffle}
\end{figure}

\subsection{Acoustic-only Deepfake Detector}\label{ssec:design_detection}
Recent studies \cite{ADD_survey,Rawformer} have indicated that the potential of Transformers in audio deepfake detection using full-information audio waveforms. In our scenario, however, the absence of semantic information combined with shuffling-induced acoustic patterns disorder (\textit{e.g.}, timbre and prosody) presents a unique challenge in detection.
\blue{To this regard, we develop a Transformer-based detector and determine its optimal number of heads for Multi-Head Self-Attention (MHSA) mechanism~\cite{vaswani2017attention}. This configuration allows the model to more effectively engage in long-range feature interaction and dynamic spatial weighting.} It adeptly captures the slight differences between bonafide and deepfake audio. Moreover, it leverages parallel computation, allowing each attention head to independently process different aspects of the input feature space. The aggregated features then form an attention spectrum, which is crucial for adaptively modulating features to more accurately detect deepfakes.
% \red{To overcome the shuffle-induced ....}
% \red{1D position encoding}

As shown in Figure~\ref{fig:bdm}, we propose the Acoustic-only Deepfake Detector (ADD), which focuses on determining the genuineness of audio by analyzing only the shuffled acoustic tokens $\mathbf{\overline{A}}$.
Specifically, we first flatten the high-frequency tones along the time and frequency axes and add positional information into $\mathbf{\overline{A}}$ using the sine and cosine alternating functions to enhance the MHSA modelling capabilities: 
\begin{align}
 \text{PE}(\mathbf{\overline{A}}, 2i)=\sin [\frac{\mathbf{\overline{A}}}{10000^{(\frac{2i}{C})}}];
 \text{PE}(\mathbf{\overline{A}}, 2i+1)=\cos [\frac{\mathbf{\overline{A}}}{10000^{(\frac{2i}{C})}}].
\end{align}
where $C$ denotes the token dimensions. We then feed $\mathbf{\overline{A}}$ into two sets of transformer encoders to process the sequence as a whole and capture global dependencies. Each set comprises two Feed-Forward Networks (FFNs), Multi-Head Self-Attention (MHSA), and Layernorm modules. The output from the Transformer encoders is finally directed to a fully connection layer, which determines whether the audio is a deepfake.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/design_transformer.pdf}
    \caption{Acoustic-only deepfake detector (\ding{174}) of \sys.}
    \label{fig:bdm}
\end{figure}

% this layer includes bottleneck feats -> 1024 tokens, and before this, we set a torch.randperm function to randomly shuffle the feats, and we find that (这里需要把shuffle的那种token替换画出来)
\subsection{Real-world Augmentation}\label{ssec:codec_augment}
It is noteworthy that the deepfake-and-bonafide gap in waveforms will be degraded by codec transformations, posing a significant challenge in distinguishing genuine from deepfake audio in real-world telecom channels. To address this challenge, we have strategically incorporated a few representative codecs into our training pipeline. These include OPUS~\cite{Opus}, known for its versatility and efficiency across audio types, and G.722~\cite{G.722}, renowned for high-quality voice transmission. We also utilize GSM for its widespread application in mobile communication, and both $\mu$-law and A-law~\cite{G.711} codecs, prevalent in North American, European, and international telephone networks. Additionally, we incorporate the MP3 codec~\cite{MP3}, a popular lossy compression technique in digital audio but introducing distortions and artifacts. Our diverse codecs integration strategy enables \sys to handle unique distortions each codec introduces and potentially generalize to more unseen coding technologies. The enhanced training process promote \sys maintains high accuracy and reliability in various real-world scenarios, where codec-induced variations are prevalent.

% We set the default configuration as \red{here we should put the hyperparameters of \sys, which can be pre-mentioned in \S.Design. An example is given below:}
% We set the default configuration as D = 41,641, Do = 32,089, N = 192, F = 1,025, K = 5, and a batchsize of 64. The l$\inf$-norm constraint, $\varepsilon$, is sampled from a normal distribution $N(\mu, \sigma)$ with the mean $\mu$ = 0.05 and the variance $\sigma$ = 0.05. Note that we randomize $\varepsilon$, the constraint value of l$\inf$ to train the Throttle module in V-CLOAK to learn to adjust the magnitude of each feature under different constraints. In the training phase, we use an Adam [23] optimizer to update the parameters of the anonymizer G for 50 epochs, with a learning rate of 4e-4. The default adversary is A1.
% more details including hyperparameters can be found in Appendix~\ref{appendix:implement_details}.

\subsection{\sys Prototype}\label{ssec:prototype}
We have implemented a prototype of \sys using Pytorch 2.1~\cite{Pytorch}. During the training phase, we initially train \sys's codec-based decoupling model on LibriSpeech dataset \cite{librispeech} utilizing four RTX 3090 GPUs (NVIDIA), adhering to the procedure outlined in Equation~\ref{eq:all_loss}. We set the training epoch to 20. The maximum learning rate was set to $4\times 10^{-4}$, and the batch size of each GPU was 20. 
To better decouple the semantic and acoustic information of the input audio, we introduce multiple loss functions, including distillation loss $\mathcal{L}_{\text{distll}}$, reconstruction loss $\mathcal{L}_{\text{rec}}$, perceptual loss $\mathcal{L}_{\text{G}}$, and $\mathcal{L}_{\text{feat}}$ implemented via a discriminator, and RVQ commitment loss $\mathcal{L}_{\text{c}}$. 
The detailed loss functions are given in Appendix~\S\ref{sec:CDM_loss}. The CDM model is trained to optimize the following loss:
\begin{equation}\label{eq:all_loss}
    \mathcal{L}_\text{total}= \lambda_{\text{d}} \mathcal{L}_{\text{distill}} + \lambda_{\text{r}} \mathcal{L}_{\text{rec}} + \lambda_{\text{G}} \mathcal{L}_{\text{G}} + \lambda_{\text{f}} \mathcal{L}_{\text{feat}} + \lambda_{\text{c}} \mathcal{L}_{\text{c}}
\end{equation}
where we set coefficients similar to HiFiGAN~\cite{kong2020hifi}, with specific values $\lambda_{\text{d}}=1, \lambda_{\text{r}}=1, \lambda_{\text{G}}=3, \lambda_{\text{f}}=3, \lambda_{\text{c}}=1$.

For the acoustic-only deepfake detector, we set the embedding dimensions to 1024, and the dropout rate in the model to 0.1. If not stated otherwise, we inverse \sys's acoustic token sequences within each 1s segment as the default shuffle approach. For the Transformer settings in the detector, we set the number of layers in the Transformer encoder to 2, the number of MHSA's heads to 8, and the positional encoding to be ``sinusoidal". We use BCE loss function and AdamW optimizer to optimize the detection model parameters with a learning rate of $3\times 10^{-4}$ and weight decay set to $1\times 10^{-4}$. Additionally, in each iteration of the training, we randomly extract a 4-second segment from speech samples and use one 3090 GPU. 

% For the decoupled codec-based model, we set the training epoch to 20. The maximum learning rate was set to $4\times 10^{-4}$, and the batch size of each GPU was 20. 

% For the pure acoustic detection model, we set the embedding dimensions to 1024, and the dropout rate in the model to 0.1. If not stated otherwise, we inverse \sys feature sequences within each 1s segment as the default shuffle approach. For the transformer settings in the detection model, we set the number of layers in the transformer encoder to 4, the number of heads in the multi-head attention to 8, and the positional embedding technique used to be ``sinusoidal". We set the number of layers in the transformer encoder to 4, the number of heads in the multi-head attention to 8, and the positional embedding technique used to be ``sinusoidal''. In the training phase of the pure sound detection model, we use BCE loss function and AdamW optimizer to optimize the detection model parameters with a learning rate of $3\times 10^{-4}$ and weight decay set to $1\times 10^{-4}$.
% We do not employ the score-level fusion in the default setting.
% The purpose of the distillation loss is to extract semantic information from the audio. We employ HuBERT \cite{hsu2021hubert} as the semantic teacher and implement two knowledge distillation strategies: continuous representation distillation and pseudo-label prediction. For continuous representation distillation, we use the average representation of all HuBERT layer outputs as the target representation of the teacher. This method allows the model to learn better and emulate the rich semantic information provided by HuBERT during training. Specifically, the training objective for continuous representation distillation can be expressed as:
% \begin{equation}
%     \mathcal{L}_{\text{distll}}=\log \sigma\left(\cos \left(\mathbf{W} \cdot q(\mathbf{z_1} ), \mathbf{H} \right)\right),
% \end{equation}
% where $q(\mathbf{z}_1)$ represents the output of the first VQ layer, $\mathbf{H}\in \mathbb{R}^{C\times T_n}$ denotes the mean of the output features of all HuBERT layers, $\cos(\cdot)$ signifies the cosine similarity between two variables, and $\mathbf{W}$ is the projection matrix.

% The reconstruction loss consists of two parts: the time domain and the frequency domain. In the time domain, the aim is to minimize the L1 distance between the target and the compressed audio to ensure accurate reconstruction in the time dimension. In the frequency domain, on the other hand, we take a more nuanced approach that involves a linear combination of L1 and L2 losses on the Mel spectrogram at different time scales. This approach aims to capture and minimize the difference in frequency characteristics between the target and generated audio. Formally, the reconstruction loss can be expressed as:
% \begin{equation}
%     \mathcal{L}_{{\text{rec}}}=\sum_{i \in e}(\left\|\mathcal{M}_{i}(\mathbf{A})-\mathcal{M}_{i}(\bar{\mathbf{A}})\right\|_{1}+\left\|\mathcal{M}_{i}(\mathbf{A})-\mathcal{M}_{i}(\bar{\mathbf{A}})\right\|_{2})+||\mathbf{A}-\bar{\mathbf{A}}||_1,
% \end{equation}
% where $\mathcal{M}_i(\cdot)$ denotes the mel spectrogram using STFT with different window sizes $2^i$ and hop sizes $2^i//4$, $i\in [5,11]$.

% We introduce the adversarial loss model to learn the features of real audio more efficiently and thus generate high-quality audio under different discriminator evaluations. This strategy not only improves the realism of the generated audio but also enhances the robustness of the model in complex audio generation tasks. Specifically, we compute the losses of multiple discriminators and perform time averaging to obtain a combined adversarial loss value. Formally, this adversarial loss can be expressed as:
% \begin{align}
%      \mathcal{L}_{{\text{G}}}&=\frac{1}{K} \sum_{k=1}^{K} \max \left(1-D_{k}(\bar{\mathbf{A}}), 0\right), \\
%     \mathcal{L}_{\text{D}}&=\frac{1}{K} \sum_{k=1}^{K} \max \left(1-D_{k}(\mathbf{A}), 0\right)+\max \left(1+D_{k}(\bar{\mathbf{A}}), 0\right),
% \end{align}
% where $K$ denotes the number of discriminators $D_k(\cdot)$. In addition, we also add a relative feature matching loss \cite{defossez2022high} to the generator:
% \begin{align}
% \mathcal{L} _{\text {feat }}(\mathbf{A} , \bar{\mathbf{A}})=\frac{1}{K L} \sum_{k=1}^{K} \sum_{l=1}^{L} \frac{\left\|D_{k}^{l}(\mathbf{A})-D_{k}^{l}(\bar{\mathbf{A}})\right\|_{1}}{\operatorname{mean}\left(\left\|D_{k}^{l}(\mathbf{A})\right\|_{1}\right)},
% \end{align}
% where $L$ denotes the number of layers in discriminators.

% For the RVQ, we introduce a computation of the commitment loss $\mathcal{L}_c$ between the pre-quantized and quantized values. Note that the quantized values do not compute the gradient. This training objective can be formulated as follows:
% \begin{equation}
%     \mathcal{L}_c=\sum_{N_q}^{i=1}\left \| \mathbf{z}_i - q(\mathbf{z}_i) \right \|^2_{2}
% \end{equation}

% In summary, the CDM model is trained to optimize the following loss:
% \begin{equation}\label{eq:all_loss}
%     \mathcal{L}_\text{total}= \lambda_{\text{distll}} \mathcal{L}_{\text{distll}} + \lambda_{\text{rec}} \mathcal{L}_{\text{rec}} + \lambda_{\text{G}} \mathcal{L}_{\text{G}} + \lambda_{\text{feat}} \mathcal{L}_{\text{feat}} + \lambda_{\text{c}} \mathcal{L}_{\text{c}},
% \end{equation}
% where we set coefficients similar to HiFiGAN, with specific values $\lambda_{\text{distll}}=1, \lambda_{\text{rec}}=1, \lambda_{\text{G}}=3, \lambda_{\text{feat}}=3, \lambda_{\text{c}}=1$.

==> sections/introduction_highlight.tex <==
% !TEX ROOT =../main.tex

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.42\textwidth]{figures/Fig1.pdf}
    \includegraphics[width=0.48\textwidth]{figures/Fig1_v2.pdf}
    \caption{\sys framework decouples and processes speech samples into semantic and acoustic information. By using acoustic-only information, \sys achieves reliable deepfake detection while protecting user content privacy from recovery attacks.}
    \label{fig:fig1}
    \vspace{-10pt}
\end{figure}
\section{Introduction}
% 深度伪造检测和用户隐私保护是两个重要问题，本文make the first attempt to提供这种解决方案。Our talk with companies convey their concerns about being not trusted by users. 尽管隐私政策声明了不会侵犯用户隐私，但是用户对各个公司的信任仍然不足，特别在商业机密场景。因此提出一种同时能满足深度伪造且从技术实现角度不会泄露用户内容隐私的方法是十分重要的。
% 可以举一些公司非法收集用户信息、内容的新闻报道，导致用户对于公司更不信任
Recent advances in text-to-speech (TTS) and voice conversion (VC) technologies have enabled the generation of highly realistic and natural-sounding speech, imitating specific individuals saying things they never actually said. However, such technologies have been misused to create audio deepfakes, posing significant security threats. 
For instance, deepfakes disseminated on the Internet can manipulate public opinion, serving purposes like propaganda, defamation, or terrorism~\cite{suwajanakorn2017synthesizing, PoliticDeepFake}.	
Besides, audio deepfake fraud in calls and virtual meetings, including a notable UK case where \$35 million was stolen using a cloned CEO's voice~\cite{CEOscam}, have affected 7.7\% of individuals financially, according to a 2023 McAfee survey~\cite{McAfeeReport}. 
These have spurred the development of diverse audio deepfake detection models~\cite{ADD_survey,AASIST,RawNet2}, designed to discern synthetic from genuine voices and promptly alert potential victims. However, existing works~\cite{AASIST,RawNet2,Rawformer,LCNN-LSTM,ASVspoof2021-baselines} typically take audio waveform or spectral features as inputs to leverage complete speech information.

% audio deepfake attackers pose fortune threats to individuals and organizations. A 2023 McAfee survey reveals that about 7.7\% of people lost money due to AI voice cloning scams~\cite{individFraud,McAfeeReport}, with cases like a UK incident where a CEO's voice was cloned to fraudulently transfer \$35 million~\cite{CEOscam}. 
% Additionally, the reliability of voice ID systems in financial contexts is under threat~\cite{VoiceID1,VoiceID2} due to the increasing sophisticated attacks.

% Application scenario of \sys. A fraudster uses audio deepfake techniques to transform their voice to sound like the target person, \textit{e.g.}, a business partner or acquaintances of the victim. \sys decouples and processes the speech sample into acoustic and semantic tokens. With only acoustic information uploaded to the detector, \sys ensures comparable anti-deepfake performance while preventing user's content privacy from exposure to the detection side.

% There is a noticeable lack of consideration for the potential privacy risks these methods pose to users.
% Despite numerous existing works on deepfake detection models that utilize audio waveforms or spectral features to leverage complete speech information, there is a noticeable lack of consideration for the potential privacy risks these methods pose to users.
Imagine a scenario where you engage in virtual calls or online meetings, potentially discussing sensitive matters like business secrets or personal health reports. While deepfake detection models are beneficial for identifying potential scams during conversations, there is hesitancy in using them due to the risk of confidential content leakage. In this paper, we introduce \sys, a novel framework designed to preserve content privacy while effectively detecting audio deepfakes. As shown in Figure~\ref{fig:fig1}, the key idea of \sys is to decouple speech into semantic and acoustic information. This approach enables reliable deepfake detection using processed acoustic information, while preventing adversaries from accessing the content, even if they employ advanced automatic speech recognition (ASR) models or direct human auditory analysis.
% Given that detecting audio deepfakes focuses on the unnatural prosody, timbre, and subtle artifacts existed in machine-synthetic speech,

To our knowledge, this is the first work to develop a content privacy-preserving audio deepfake detection framework. \sys is inspired by an insightful intuition that audio deepfakes aim to replicate a speaker's timbre and prosody, while disregarding the content, \textit{i.e.}, acoustic-centric. In contrast, speech recognition systems focus on extracting semantic content, independent of the speaker-related features, \textit{i.e.}, semantic-centric. This dichotomy indicates that these two tasks may rely on mutually independent features, suggesting the potential for designing an effective audio deepfake detector analyzing only acoustic information without exposing semantic content. 
% The idea sounds promising yet challenging, exemplified by the following two questions.
However, materializing \sys sounds promising yet challenging in two aspects.

% To our knowledge, this is the first work to develop a content privacy-preserving audio deepfake detection framework. \sys reliably monitors deepfakes in everyday virtual communications without exposing actual user dialogues. The idea sounds promising yet challenging. First of all, \sys must safeguard content privacy against both machine-based and human auditory analysis. Prior works using adversarial examples~\cite{carlini2018audio,li2024vrifle} for ASR model disruption or speaker anonymization~\cite{deng2023v,o2022voiceblock,miao2023speaker} have shown limited effectiveness against human listeners. 
% Secondly, \sys has to deliver accurate detection of various real-world deepfakes, even with limited speech information post-disentanglement. Unlike prior models that utilize raw waveforms, spectral features, and pretrained representation inputs---thus compromising user privacy---\sys seeks to achieve comparable results using only acoustic information. To address these challenges, we answer the following two questions.

%1. 我们不能仅仅防御模型，也要防御人，因为人也可能会听内容，不能仅仅用一些对抗样本的方法去对抗机器，必须实现两者都不能听；但是做密码学操作又很慢，要有一定实时性. 此外我们，对特征序列进行混淆，进一步打破时序依赖
% 2. 如何仅基于信息缺失的状态进行可靠的deepfake检测？通过
% 3. 

% 用户不仅要防御机器偷听声音，还要防止检测方可能有人为的窃听（如先将特征复原为音频，再窃听）
\textbf{Content Protection.} \textit{How to protect content privacy from recovery by adversaries?}
\sys aims to safeguard speech content privacy against both machine-based and human auditory analysis. Prior works using adversarial examples~\cite{carlini2018audio,li2024vrifle} for ASR model disruption or speaker anonymization~\cite{deng2023v,o2022voiceblock,miao2023speaker} have shown limited effectiveness against human listeners. \sys tackles this by decoupling speech into semantic and acoustic tokens and provides only the acoustic tokens to the detector, where tokens means the discrete representations of information. Consequently, although content recovery adversaries can receive a series of acoustic tokens, the scant semantic cues hinder their recovery of understandable content. This approach, along with randomly shuffling the acoustic tokens, further obfuscates the contextual patterns that both machine-based and human auditory analysis rely on for content comprehension. \sys also defends against a range of adversaries who might use decoders to transform anonymized acoustic tokens into speech waveforms and analyze them.
% 主要通过codec增强+transformer结构，我们还证明了SafeEar前端架构可以适配其他主流的deepfake检测分类器，如GNN.


% 在这里就应该把key observation讲清楚，为什么我们觉得缺少语义信息的deepfake detection可以做？
\textbf{Deepfake Detection.} \textit{How to deliver accurate deepfake detection merely based on acoustic tokens?}
The challenge lies in the absence of semantic information and the disrupted acoustic patterns (\textit{e.g.}, timbre and prosody) due to shuffling. These content protection strategies may complicate the identification of cues necessary to differentiate genuine from synthetic audio. We address this by designing a dual-augmentation strategy in our transformer-based detector, comprising a multi-head self-attention (MHSA) mechanism and positional encoding. This allows the deepfake detector to capture dynamic spatial weighting and local-global feature interactions. Additionally, deepfakes can occur across various communication platforms, which are transmitted via different telecom channels. This can degrade the deepfake-and-genuine gap due to the effects of codec compression during telecom.
To address this, we strategically integrated several representative codecs into our training pipeline to counteract the disruptive effects of codec transformation, ensuring high accuracy and reliability across diverse real-world scenarios. % Apart from Transformer, we also validate that \sys can cooperate with different detectors as backend.
% the above challenge that  nullifies content recovery attempts, has little adverse impact on our deepfake detection task.
% Given that detecting audio deepfakes focuses on the unnatural prosody, timbre, and subtle artifacts existed in machine-synthetic speech,
% This operation benefits our detection approach to be content- and language-independent, where the time series disorder severely affects ASR should not impact our system.
% The robustness of our detection approach is content- and language-independent, meaning the time series disorder that severely affects Automatic Speech Recognition (ASR) should not impact our system. 
% To counter this, we have integrated several representative codecs into our training process, enhancing the system’s resilience against codec transformations. Despite these potential disturbances, the augmented training ensures that \sys achieves high accuracy and reliability across diverse real-world scenarios. Our validations confirm that \sys is compatible with various detector backends.
% Moreover, we present positional encoding for better capturing local-gloabl dependency, especially consider the input features are disordered, which can severally disrupt the continual paralinguistic features (\textit{i.e.}, timbre and prosody), we encourage the local-global capturing ability of position encoding combined with the MHSA can largely alleviate the disorder affects on deepfake detection. 
% This is comprehensible because the deepfake detection is content- and language-independent, \textit{i.e.}, the disorder of time series that affects ASR severally should not affect it. 

\textbf{Benchmark Construction.}
We construct a comprehensive benchmark to evaluate systems for deepfake detection and content privacy protection. This benchmark comprises four datasets, including three standard datasets (ASVspoof 2019 and ASVspoof 2021 for deepfake detection, and Librispeech for content protection), and CVoiceFake---our established multilingual dataset sourced from the CommonVoice dataset. CVoiceFake, with over 1.25 million voice samples in five languages generated using five representative deepfake generation techniques, also includes ground-truth textual transcriptions, making it also an ideal benchmark against content recovery attacks. To our knowledge, CVoiceFake fills a gap in cross-language deepfake datasets~\cite{ADD_survey} and we hope it can serve as a basis for future research developments.

\textbf{Extensive Evaluation.}
Our extensive experiments, based on the above benchmark datasets, focus on two critical tasks: deepfake detection and content protection. 
For the deepfake detection task, we benchmark \sys against eight baseline detectors across three deepfake datasets featuring a variety of deepfake speech samples generated using popular TTS and VC technologies. This task also considers impact factors like different transmission channels, and languages.
Regarding the content protection task, we evaluate \sys's efficacy against three levels of content recovery adversaries: \textit{naive} (CRA1), \textit{knowledgeable} (CRA2), and \textit{adaptive} (CRA3). \sys demonstrates robustness in safeguarding speech content in English and four extra unseen languages, effectively hindering CRA1 from using leading ASR architectures to interpret acoustic tokens, preventing CRA2 from exploiting \sys's decoder to reconstruct speech waveforms for machine-based and human auditory analysis, and thwarting CRA3's efforts to reorder shuffled token sequences for further analysis. Our experiments show that \sys achieves comparable performance with top-tier deepfake detectors based solely on acoustic information, with an optimal equal error rate (EER) as low as 2.02\%. Moreover, \sys effectively defends against content recovery attempts by adversaries, maintaining all word error rates (WERs) to above 93.9\%.


\textbf{Summary of Contributions.} Our technical and experimental contributions are as follows:
\begin{icompact}
    \item To our knowledge, we make the first attempt to investigate the feasibility of achieving precise audio deepfake detection while preserving user content privacy, which may promote privacy-centric intelligent services.
    
    \item We propose \sys, a novel privacy-preserving deepfake detection framework that devises the neural audio codec into a semantic-acoustic information decoupling model, which ensures the content privacy. We further develop an advanced detector performs effective detection with only acoustic information.

    \item We establish a comprehensive benchmark focusing on deepfake detection and content privacy preservation. Our extensive comparison experiments demonstrate \sys's robust effectiveness in diverse scenarios. Moreover, \sys effectively resists multiple content recovery attacks.
    
    % based on which we verify the effectiveness of \sys compared with multiple baseline methods.
    
    % \item We make the first attempt to design \sys, a decoupling-and-detection framework that can achieve ideal performance on audio deepfake mitigation while protecting user's content privacy. \sys complement and seamlessly integrate with widely-used codecs, and can generalize to different languages.

    % \item We conduct extensive experiments for evaluating \sys on 6 speech datasets and 5 languages, from which we verify the effectiveness of our method compared with existing works and see a new paradigm of privacy-preserving deepfake detection.
\end{icompact}


==> sections/shuffle_algorithm.tex <==
\section{Innumerable Shuffle Combinations}\label{appendix:shuffle_proof}

The core premise of the shuffle algorithm, as implemented in \sys, revolves around the principle of creating a high level of uncertainty in the temporal sequence of acoustic tokens. This is achieved by employing a random rearrangement strategy within specified intervals (1-second windows or 50 frames). The proof of the algorithm's robustness against reconstruction attempts lies in the combinatorial complexity introduced by this randomization process.

For a given 1-second window of 50 frames, the number of possible permutations is $50!$ (50 factorial), which is approximately $3.0414 \times 10^{64}$. This factorial growth rate results in an astronomically high number of possible frame arrangements. Even if an adversary were to attempt reconstructing the original sequence, the probability of correctly guessing the exact order of just one 50-frame window is $1$ in $3.0414 \times 10^{64}$, which is virtually impossible for practical purposes.

Moreover, considering the entire sequence of acoustic tokens $\mathbf{A}^{b} \in \mathbb{R}^{C\times T_n}$, where $T_n$ represents the total number of temporal frames, the complexity magnifies. Assuming the total number of frames is a multiple of 50, the number of potential permutations across the entire sequence becomes:
\begin{equation}
P_{total} = (50!)^{T_n/50}
\end{equation}
This value represents the total number of unique ways the entire sequence could be arranged, further exacerbating the challenge for any attempt at reconstruction.

In probabilistic terms, the chance of accurately reconstructing the shuffled acoustic token sequence $\mathbf{\overline{A}}$ to correct-order $\mathbf{A}$ diminishes exponentially with each additional 50-frame window:
\begin{equation}
P_{\mathbf{A}} = \left(\frac{1}{50!}\right)^{T_n/50}
\end{equation}
Even with advanced computational resources, the task of aligning these permutations to derive intelligible speech content becomes computationally infeasible. This combinatorial explosion ensures that the shuffling process effectively protects against content recovery, as adversaries face insurmountable odds in aligning the shuffled frames to their original sequence.

Thus, the shuffle algorithm within \sys serves as a formidable barrier against content recovery attempts. By leveraging the principles of combinatorics and probability, the algorithm ensures that any attempt at reconstructing the original speech sequence from the shuffled frames remains a highly improbable endeavor, thereby upholding the integrity of content protection in \sys.



==> tables/10_Librispeech_API_adaptive.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[ht]\centering
\small
\renewcommand{\arraystretch}{0.8} 
% \resizebox{0.85\linewidth}{!}{
% \begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\tabcolsep}{2.5pt}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[T2] Protecting English content from \textit{adaptive adversary}’s recovery attacks (CRA3).}
\begin{tabular}{llcccc}
\toprule[1.2pt]
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ASR Model}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Input}}} & \multicolumn{2}{c}{\textbf{Libri. test-clean}} & \multicolumn{2}{c}{\textbf{Libri. test-other}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & WER (\%)$\uparrow$ & CER (\%)$\uparrow$ & WER  (\%)$\uparrow$ & CER (\%)$\uparrow$ \\
\midrule[1pt]
Wav2Vec2 & \sys & 92.58 & 60.81 & 99.01 & 69.12 \\
\midrule
Iflytek API & \sys & 92.40 & 72.56 & 98.50 & 77.16 \\
\midrule
 
Tecent API & \sys & 87.46 & 81.86 & 92.23 & 87.89 \\
\midrule

Azure API & \sys & 92.94 & 89.20 & 96.04 & 92.87 \\
\midrule

Amazon API & \sys & 82.73 & 71.80 & 90.44 & 80.60 \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:test_speech_libri_ASR_adaptive}
\end{table}

==> tables/11_commonvoice_API_adaptive.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[ht]\centering
\small
\renewcommand{\arraystretch}{0.8} 
% \resizebox{0.85\linewidth}{!}{
% \begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\tabcolsep}{3pt}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[T2] Cross-language content protection from \textit{adaptive adversary}’s recovery attacks (CRA3).}
\begin{tabular}{llccccc}
\toprule[1.2pt]
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ASR Model}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Input}}} & \multicolumn{5}{c}{\textbf{CVoiceFake  WER (\%)}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & English & Chinese & German & French & Italian \\
\midrule[1pt]
\multirow{1}{*}{Wav2Vec2} & \sys & 97.28 & 73.29 & 104.02 & 96.46 & 101.51 \\
\midrule
\multirow{1}{*}{Iflytek API} & \sys & 100.4 & 85.06 & 94.58 & 114.81 & 98.45 \\
\midrule
\multirow{1}{*}{Tencent API} & \sys & 86.27 & 76.93 & - & 81.95 & - \\
\midrule
\multirow{1}{*}{Azure API} & \sys & 94.72 & 78.55 & 93.46 & 94.95 & 92.30 \\
\midrule
\multirow{1}{*}{Amazon API} & \sys & 91.67 & 86.73 & 81.48 & 78.68 & 83.31 \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:test_speech_commonvoice_ASR_adaptive}
\end{table}

==> tables/13_additional_cost.tex <==
\begin{table}[t!]
\centering
\small
\renewcommand{\arraystretch}{1} 
% \resizebox{0.85\linewidth}{!}{
% \begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\tabcolsep}{6pt}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
\color{blue}
\caption{\label{tab:additional_cost}Additional cost of \sys compared with baseline methods: RTF and FLOPs.}
\begin{threeparttable}
\begin{tabular}{@{}llcc@{}}
\toprule[1.2pt]
\multicolumn{1}{c}{\textbf{Type}} & \multicolumn{1}{c}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{RTF} $\downarrow$} & \multicolumn{1}{c}{\textbf{FLOPs} $\downarrow$} \\
\midrule[1pt]
\multirow{2}{*}{\textbf{End-to-End}}   & AASIST  &  0.0155  &  45.49T  \\
& Rawformer   &   0.0145   &  5.24T  \\
\midrule
\multirow{2}{*}{\textbf{Pipeline}}        & Wav2vec2+Transformer   &    0.0111   &  47.05T  \\
& SafeEar (Ours)   &   0.0366  &  62.76T  \\
\bottomrule[1.2pt]
\end{tabular}
% \begin{tablenotes}[flushleft]
%     \item[] \vspace{-2pt}\hspace{-2pt}\small 
%     (1) $^\natural$: RTF is short for ``Real-Time Factor'', RTF=$T_{detect}$/$T_{audio}$, indicating how fast the model can process audio input, where $T_{audio}$ is the duration of the original audio, and $T_{detect}$ is the time to detect the authenticy of the audio.\\
%     (2) $\ddagger$: FLOPs quantify the number of floating point operations, is hardware-agnostic metric to compare the inherent computational demands of different models, the lower the FLOPs, the lower the algorithmic complexity the model has.
% \end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/7_Librsispeech_API.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t!]\centering
\small
\renewcommand{\arraystretch}{0.8} 
% \resizebox{0.85\linewidth}{!}{
% \begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\tabcolsep}{3pt}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[T2] Protecting English content from \textit{knowledgeable adversary}’s recovery attacks (CRA2).}
\begin{tabular}{llcccc}
\toprule[1.2pt]
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ASR Model$^\ddagger$}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Input$^\natural$}}} & \multicolumn{2}{c}{\textbf{Libri. test-clean}} & \multicolumn{2}{c}{\textbf{Libri. test-other}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & WER (\%)$\uparrow$ & CER (\%)$\uparrow$ & WER  (\%)$\uparrow$ & CER (\%)$\uparrow$ \\
\midrule[1pt]
\multirow{3}{*}{Wav2Vec2} & Original & 3.15 & 0.88 & 7.68 & 2.72 \\
 & All Info & 3.82 & 1.17 & 11.83 & 4.86 \\
 & \cellcolor{lightgray}\textbf{\sys} & \cellcolor{lightgray}\textbf{101.1} & \cellcolor{lightgray}91.99 & \cellcolor{lightgray}\textbf{101.46} & \cellcolor{lightgray}93.19 \\
\midrule
 
\multirow{3}{*}{Iflytek API} & Original & 8.09 & 4.25 & 13.80 & 6.94 \\
 & All Info & 17.82 & 14.18 & 24.36 & 16.71 \\
 & \cellcolor{lightgray}\textbf{\sys} & \cellcolor{lightgray}98.59 & \cellcolor{lightgray}93.10 & \cellcolor{lightgray}99.54 & \cellcolor{lightgray}93.62 \\
\midrule
 
\multirow{3}{*}{Tecent API} & Original & 4.65 & 3.07 & 8.14 & 4.56 \\
 & All Info & 14.74 & 13.13 & 18.56 & 14.12 \\
 & \cellcolor{lightgray}\textbf{\sys} & \cellcolor{lightgray}99.52 & \cellcolor{lightgray}99.40 & \cellcolor{lightgray}99.68 & \cellcolor{lightgray}99.62 \\
\midrule
 
\multirow{3}{*}{Azure API} & Original & 5.14 & 3.25 & 10.58 & 6.43 \\
 & All Info & 5.68 & 3.51 & 14.56 & 8.95 \\
 & \cellcolor{lightgray}\textbf{\sys} & \cellcolor{lightgray}100.0 & \cellcolor{lightgray}\textbf{99.98} & \cellcolor{lightgray}100.0 & \cellcolor{lightgray}\textbf{100.0} \\
\midrule
\multirow{3}{*}{Amazon API} & Original & 4.98 & 3.24 & 8.56 & 4.80 \\
 & All Info & 15.00 & 13.33 & 19.06 & 14.25 \\
 & \cellcolor{lightgray}\textbf{\sys} & \cellcolor{lightgray}99.86 & \cellcolor{lightgray}95.54 & \cellcolor{lightgray}99.70 & \cellcolor{lightgray}95.07\\ 
% \multirow{3}{*}{Google API} & Original & 14.83 & 8.23 & 29.56 & 18.01 \\
%  & All Info & 24.41 & 17.85 & 39.47 & 27.65 \\
%  & \sys & 99.48 & 98.64 & 98.69 & 97.33\\
\bottomrule[1.2pt]
\end{tabular}
\begin{tablenotes}[flushleft]
    \item[] \vspace{-2pt}\hspace{-2pt}\small 
    (i) $\ddagger$: Here Wav2Vec2 denotes the open-source ASR model~\cite{facebook_wav2vec2}.
    (ii) $\natural$: \textit{Original} means uncompressed audio; \textit{Coded} means the audio is reconstructed by combining semantic and acoustic tokens.
\end{tablenotes}
\label{tab:test_speech_libri_ASR}
\end{table}

==> tables/dataset.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]\centering
% \scriptsize
\renewcommand{\arraystretch}{1} 
% \resizebox{0.85\linewidth}{!}{
% \begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\tabcolsep}{6pt}
% \setlength{\abovecaptionskip}{0pt}% 
% \setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{Dataset Statistics.}
\begin{tabular}{@{}l|l|l|l|l|l|l@{}}
\toprule
\textbf{Task}                  & \textbf{Dataset} & \textbf{Character} & \textbf{Language} & \textbf{Train Samples}      & \textbf{Test Samples}  & \textbf{Duration (s)} \\ \midrule
\multirow{2}{*}{Anti-Deepfake} & ASVspoof 2019    & clean              & English           & B: 2,580  D: 22,800         & B: 7,355 D: 63,882     & 0.47$\sim$16.55       \\ \cmidrule(l){2-7} 
                               & ASVspoof 2021    & telecom codec      & English           & B: 2,580  D: 22,800         & B: 14,816 D: 133,360   & 0.36$\sim$13.40       \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Anti-Deepfake\\ \\  \&\\ \\ Anti-Content\\ Recovery\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CVoiceFake\\ (Multilingual)\end{tabular}} &
  \multirow{5}{*}{media codec} &
  English &
  B: 34,521  D: 171,544 &
  B: 8,630 D: 42,886 &
  0.97$\sim$10.69 \\ \cmidrule(l){4-7} 
                               &                  &                    & Chinese           & B: 34,421  D: 168,872       & B: 8,605 D: 42,218     & 1.51$\sim$19.66       \\ \cmidrule(l){4-7} 
                               &                  &                    & German            & B: 32,000  D: 159,301       & B: 8,000 D: 39,826     & 1.48$\sim$11.12       \\ \cmidrule(l){4-7} 
                               &                  &                    & French            & B: 38,584 D: 188,897        & B: 9,646 D: 47224      & 0.79$\sim$11.81       \\ \cmidrule(l){4-7} 
                               &                  &                    & Italian           & B: 29822  D: 145,952        & B: 7,456 D: 36,488     & 0.79$\sim$14.11       \\ \midrule
Anti-Content Recovery          & LibriSpeech      & clean              & English           & \multicolumn{1}{r|}{28,539} & Dev: 2,703 Test: 2,620 & 1.29$\sim$34.96       \\ \bottomrule[1.2pt]
\end{tabular}
\label{tab:test_overall_sexual}
% \end{threeparttable}}
\end{table*}
